Assessing Sensitivity of Machine Learning Predictions.A Novel Toolbox with an Application to Financial Literacy

Despite their popularity, machine learning predictions are sensitive to potential unobserved predictors. This paper proposes a general algorithm that assesses how the omission of an unobserved variable with high explanatory power could affect the predictions of the model. Moreover, the algorithm extends the usage of machine learning from pointwise predictions to inference and sensitivity analysis. In the application, we show how the framework can be applied to data with inherent uncertainty, such as students' scores in a standardized assessment on financial literacy. First, using Bayesian Additive Regression Trees (BART), we predict students' financial literacy scores (FLS) for a subgroup of students with missing FLS. Then, we assess the sensitivity of predictions by comparing the predictions and performance of models with and without a highly explanatory synthetic predictor. We find no significant difference in the predictions and performances of the augmented (i.e., the model with the synthetic predictor) and original model. This evidence sheds a light on the stability of the predictive model used in the application. The proposed methodology can be used, above and beyond our motivating empirical example, in a wide range of machine learning applications in social and health sciences.

==> Tables/Discriptive_Results.tex <==
\begin{table}[H]
\caption{Summary Statistics of the Sub Sample (Normal and Low FLS) Predictors}
\label{tablesummarystats}
\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\begin{tabular}{l*{3}{D{.}{.}{-1}}}
\toprule \addlinespace
                & Normal FLS&         &         & Low FLS&         &         &Difference in Means\\ \addlinespace
                &     Mean&       SD&        N&     Mean&       SD&        N&  p-value\\
\midrule
\               &         &         &         &         &         &         &         \\
\addlinespace
\textit{Student Characteristics}&         &         &         &         &         &         &         \\
\addlinespace
International Grade&     3.31&     2.16&     8277&     6.07&     1.69&     1374&    0.000\\
\addlinespace
Gender          &     1.50&     0.50&     8277&     1.54&     0.50&     1347&    0.003\\
\addlinespace
Age             &    15.89&     0.31&     8277&    15.87&     0.33&     1374&    0.080\\
\addlinespace
Study Track: ISCED Designation &     2.22&     0.63&     8277&     3.15&     0.92&     1374&    0.000\\
\addlinespace
Study Track: ISCED Orientation &     3.15&     1.46&     8277&     4.22&     1.31&     1374&    0.000\\
\addlinespace
Speaks Belgian Language at Home&     2.06&     0.28&     8277&     2.31&     0.51&     1374&    0.000\\
\addlinespace
\               &         &         &         &         &         &         &         \\
\textit{Socioeconomic Status}&         &         &         &         &         &         &         \\
\addlinespace
Educational Resources at Home&     0.19&     0.88&     8277&    -0.43&     1.05&     1374&    0.000\\
\addlinespace
Family Wealth Index (Economic Possessions) &     0.18&     0.76&     8277&    -0.05&     1.01&     1374&    0.000\\
\addlinespace
Number of Books at Home&     4.58&     1.77&     8277&     3.44&     1.81&     1374&    0.000\\
\addlinespace
Immigration Status&     3.01&     0.36&     8277&     2.95&     0.63&     1374&    0.000\\
\addlinespace
Mother's Education (ISCED)&   6.45&     1.40&     8277&     6.14&     1.70&     1374&    0.000\\
\addlinespace
Father's Education (ISCED)&     6.22&     1.42&     8277&     6.01&     1.66&     1374&    0.000\\
\addlinespace
Mother's Job (ISEI)&    47.51&    22.34&     8277&    31.54&    18.99&     1374&    0.000\\
\addlinespace
Father's Job (ISEI)&    46.75&    21.67&     8277&    33.96&    16.92&     1374&    0.000\\
\addlinespace
Parents Emotional Support&    0.01&     0.95&     8277&     -0.19&     1.07&     1374&    0.000\\
\addlinespace
\               &         &         &         &         &         &         &         \\
\textit{Achievement and Attitude}&         &         &         &         &         &         &         \\
\addlinespace
Plausible Value 1 in Mathematics&   534.24&    79.43&     8277&   367.89&    53.55&     1374&    0.000\\
\addlinespace
Plausible Value 1 in Reading&   528.54&   79.14&     8277&   345.67&    52.15&     1374&    0.000\\
\addlinespace
Grade Repetition&     2.25&     0.43&     8277&     2.80&     0.40&     1374&    0.000\\
\addlinespace
Out-of-School Study Time per Week&    14.83&    10.77&     8277&    18.27&    13.36&     1374&    0.000\\
\addlinespace
Mathematics Learning Time at School&   207.18&    76.91&     8277&   159.04&    126.93&     1374&    0.000\\
\addlinespace
Language Learning Time at School&   204.13&    75.97&     8277&   191.62&    137.84&     1374&    0.000\\
\addlinespace
Personality: Test Anxiety&    -0.21&     0.97&     8277&    -0.04&     1.15&     1374&    0.000\\
\addlinespace
Achievement Motivation&    -0.51&     0.84&     8277&    -0.32&     1.01&     1374&    0.000\\
\addlinespace
\               &         &         &         &         &         &         &         \\
\textit{School Characteristics}&         &         &         &         &         &         &         \\
\addlinespace
School Community (Location)&     5.03&     1.25&     8277&     4.53&     1.37&     1374&    0.000\\
\addlinespace
Share of Students With a Different Heritage Language&    16.87&    23.99&     8277&    35.73&    32.54&     1374&    0.000\\
\addlinespace
Share of Students With Special Needs&    15.96&    15.76&     8277&    36.98&    36.98&     1374&    0.000\\
\addlinespace
Share of Socioeconomically Disadvantaged Students &    20.15&    21.62&     8277&    52.02&    32.49&     1374&    0.000\\
\addlinespace
School Size     &   753.08&   326.03&     8277&   548.48&   302.44&     1374&    0.000\\
\addlinespace
Class Size      &    20.13&     4.40&     8277&    17.32&     5.70&     1374&    0.000\\
\addlinespace
Number of Available Computers per Student&     0.92&     0.79&     8277&     0.98&     0.93&     1374&    0.000\\
\addlinespace
Teacher Professional Development&     0.07&     0.96&     8277&     0.27&     1.04&     1374&    0.000\\
\addlinespace
School Autonomy &     0.70&     0.21&     8277&     0.68&     0.22&     1374&    0.000\\
\addlinespace
Shortage of Educational Material&     0.09&     0.88&     8277&     0.23&     0.85&     1374&    0.000\\
\addlinespace
Student-Teacher Ratio&     9.44&     2.97&     8277&     7.29&     4.25&     1374&    0.000\\
\bottomrule
\end{tabular}
\begin{tablenotes} 
\item \footnotesize{\textit{Note:} Summary statistics of all predictors used in the analysis from the PISA 2015 data for sub samples with normal and Low FLS. Low is defined as having a FLS two standard deviations smaller than the median. SD stands for the standard deviation of the variable. The last column shows the p-value of a two-sample t-test for the equality of means across the the sub samples.}
\end{tablenotes}
\end{threeparttable}


}
\end{table}

==> Tables/variables.tex <==
\begin{table}[H]
\centering
\caption{Variables Used From the PISA Data}
\label{tablevariables}
\resizebox{0.6\textwidth}{!}{%
%\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule \addlinespace
\multirow{\textit{Student Characteristics}}  \\ 
ST001D01T         & International Grade                     \\
ST004D01T         & Gender           \\
AGE               & Age  \\
ISCEDD            & Study Track: ISCED Designation                   \\
ISCEDO            & Study Track: ISCED Orientation                    \\
BELANGN           & Speaks Belgian Language at Home    \\   \addlinespace
\multirow{\textit{Socioeconomic Status}}       \\  
HEDRES            & Educational Resources at Home    \\
WEALTH            & Family Wealth Index (Economic Possessions)        \\
ST013Q01TA        & Number of Books at Home  \\
IMMIG             & Immigration Status               \\
MISCED            & Mother's Education (ISCED)             \\
FISCED            & Father's Education (ISCED)           \\
BMMJ1             & Mother's Job (ISEI)                 \\
BFMJ2             & Father's Job (ISEI)          \\
 EMOSUPS           & Parents Emotional Support      \\  \addlinespace
\multirow{\textit{Achievement and Attitude}}     \\  
PV1MATH           & Plausible Value 1 in Mathematics        \\
PV1READ           & Plausible Value 1 in Reading           \\
REPEAT            & Grade Repetition  \\
OUTHOURS          & Out-of-School Study Time per Week  \\
MMINS             & Mathematics Learning Time at School           \\
LMINS             & Language Learning Time at School              \\
ANXTEST           & Personality: Test Anxiety      \\
 MOTIVAT           & Achievement Motivation            \\   \addlinespace
\multirow{\textit{School Characteristics}}    \\  
SC001Q01TA        & School Community (Location)    \\
SC048Q01NA   & Share of Students With a Different Heritage Language \\
SC048Q02NA        & Share of Students With Special Needs          \\ 
SC048Q03NA & Share of Socioeconomically Disadvantaged Students  \\
SCHSIZE           & School Size             \\
CLSIZE            & Class Size                           \\
RATCMP1           & Number of Available Computers per Student      \\
 LEADPD            & Teacher Professional Development           \\
SCHAUT            & School Autonomy                 \\
EDUSHORT          & Shortage of Educational Material       \\
 STRATIO           & Student-Teacher Ratio                     \\ \addlinespace
\bottomrule
\end{tabular}%
}
\end{table}

==> extras.tex <==
% From the main text

% Details on the variable creation
Let us show in detail how to compute the synthetic predictor. We start from sampling $N$ independent realizations from a normally distributed continuous variable: $\tilde{R} \sim \mathcal{N}(0,1)$.\footnote{The distribution of this variable mimics the distribution of the synthetic predictor and can be directly changed by the researcher.} 
We define $\tilde{\mathbf{R}}$ the $N \times (P+2)$ matrix that stacks the output vector $Y$, $\tilde{R}$ and the matrix of observed variables $\mathbf{X}$ such that:
\begin{equation}
    \tilde{\mathbf{R}}_{(N\times (P+2))} = \big[Y_{(N \times 1)} \:\: \tilde{R}_{(N\times 1)} \:\: \mathbf{X}_{(N\times P)} \big].
\end{equation}
We define with $\hat{\mathbf{K}}$ the estimated correlation matrix of $\tilde{\mathbf{R}}$:
\begin{equation}
\hat{\mathbf{K}}_{((P+2)\times (P+2))} = 
\begin{pmatrix}
    1 & \hat{\rho}(Y,\tilde{R}) &  \ldots & \hat{\rho}(Y,X_p) \\
    \hat{\rho}(\tilde{R},Y) & 1 &  \ldots &  \hat{\rho}(\tilde{R}, X_p) \\
    \vdots & \vdots & \ddots & \vdots \\
    \hat{\rho}(X_p, Y) & \hat{\rho}(X_p, \tilde{R}) & \ldots & 1
\end{pmatrix}
\end{equation}
and with $\tilde{\mathbf{\Sigma}}= diag(\hat{\sigma}_{\tilde{Y}}^2, \hat{\sigma}_{\tilde{R}}^2, \hat{\sigma}_{X_1}^2 ..., \hat{\sigma}_{X_p}^2)$ the $(P+2) \times (P+2)$ diagonal matrix of estimated variances, where $\hat{\sigma}_{\tilde{Y}}^2$ is the estimated variance of the output, $\hat{\sigma}_{\tilde{R}}^2$ is the estimated variance of $\tilde{R}$ and $\hat{\sigma}_{\tilde{X_j}}^2$ is the estimated variance of the $j$-th variable in $\bX$. Moreover, if we define with $\mathbf{C}$ the symmetric, idempotent centering matrix:
\begin{equation}
    \mathbf{C}_{(N \times N)} = \mathbf{I}_{(N \times N)} - \frac{1}{N} \mathbf{1}_{(N \times N)}
\end{equation}
where $\mathbf{1}$ is a $N\times N$ matrix of 1s, we can center and scale the $\mathbf{\tilde{R}}$ matrix as follows:
\begin{equation}
    \dot{\mathbf{R}}_{(N \times ((P+2)))} =  \mathbf{C}_{(N \times N)} \tilde{\mathbf{R}}_{(N\times (P+2))} \tilde{\mathbf{\Sigma}}_{((P+2) \times (P+2))}^{-1}
\end{equation}
where $\dot{\mathbf{R}}_{(N \times (P+2))}$ is a multivariate normal matrix. This is similar to the type of scaling used, for example, in standard normal variate correction \citep{barnes1989standard}.
Then, we introduce no-correlation within the columns in $\tilde{\mathbf{R}}_{(N\times (P+2))}$ using the inverse of the Cholesky decomposition\footnote{This is possible as far as $\mathbf{K}$ is a symmetric positive-definite matrix.}:
\begin{equation}
    \dot{\mathbf{R}}_{(N \times (P+2))}( \mathbf{L}_{((P+2) \times 1)}\mathbf{L}_{(1 \times (P+2))}^T)^{-1}
\end{equation}
where $\mathbf{L}$ is a lower triangular matrix obtained thought the Cholesky decomposition of $\tilde{\mathbf{K}}_{((P+2)\times (P+2))}$:
\begin{equation}
    \tilde{\mathbf{K}}_{((P+2)\times (P+2))} = \mathbf{L}_{((P+2) \times 1)}\mathbf{L}^T_{(1 \times (P+2))}.
\end{equation}
The matrix that we obtain is a set of realizations of uncorrelated multivariate normal random variables. At this point, we can reintroduce the correlation between each column:
\begin{equation}
    \dot{\mathbf{R}}_{(N \times (P+2))}( \mathbf{L}_{((P+2)\times 1)} \mathbf{L}^T_{(1 \times (P+2))} )^{-1} \mathbf{U}_{((P+2)\times 1)} \mathbf{U}^T_{(1\times (P+2))}  
\end{equation}
where $\mathbf{L}$ is obtained thought as the Cholesky decomposition of $\mathbf{K}$:
\begin{equation}
  \mathbf{K}_{((P+2)\times (P+2))} = \mathbf{U}_{((P+2)\times 1)} \mathbf{U}^T_{(1 \times (P+2))}  
\end{equation}
and $\mathbf{K}$ is a newly defined correlation matrix:
\begin{equation}
\mathbf{K}_{((P+2)\times (P+2))} = 
\begin{pmatrix}
    1 & \widetilde{\rho}(Y,R) &  \ldots & \hat{\rho}(Y,X_p) \\
    \widetilde{\rho}(R,Y) & 1 &  \ldots & \widetilde{\rho}(R, X_p) \\
    \vdots & \vdots & \ddots & \vdots \\
    \hat{\rho}(X_p, Y) & \widetilde{\rho}(X_p, R) & \ldots & 1
\end{pmatrix}
\end{equation}
where $\widetilde{\rho}(Y,R)$ is the correlation between the synthetic predictor $R$ and the outcome, that is set directly by the researcher, and $\widetilde{\rho}(X_j,R)$ is the correlation between the synthetic predictor the $j-$th regressor (equal to zero in our setting):
\begin{equation}
\mathbf{K}_{((P+2)\times (P+2))} = 
\begin{pmatrix}
    1 & \widetilde{\rho}(Y,R) &  \ldots & \hat{\rho}(Y,X_p) \\
    \widetilde{\rho}(R,Y) & 1 &  \ldots & 0 \\
    \vdots & \vdots & \ddots & \vdots \\
    \hat{\rho}(X_p, Y) & 0 & \ldots & 1
\end{pmatrix}
\end{equation}
Finally, we can scale the data back to their original distribution:
\begin{equation}
    \mathbf{R}_{(N \times (P+2))}=\mathbf{C}^{-1}_{(N \times N)}\dot{\mathbf{R}}_{(N \times (P+2))}( \mathbf{L}_{((P+2)\times 1)} \mathbf{L}^T_{(1 \times (P+2))} )^{-1} \mathbf{U}_{((P+2)\times 1)} \mathbf{U}^T_{(1\times (P+2))}   \tilde{\mathbf{\Sigma}}_{((P+2) \times (P+2))}
\end{equation}
and ``extract" the newly generated synthetic predictor $R$ from the $\mathbf{R}$ matrix.  In this specific case, the synthetic predictor corresponds to the second column of the matrix $\mathbf{R}$. However, its relative position depends on how the matrix $\tilde{\mathbf{R}}$ is generated. 

At this point, we can rework the model in (\ref{formula:BART}) to include the set of stack predictors $\mathbf{G}$:
\begin{equation}\label{eq:bart_synth}
     \sum_{l=1}^{L} \mathcal{T}_l(\mathbf{G}; \mathcal{D}_l, \mathcal{M}_l) + \psi
\end{equation}
where $\mathbf{G}$ is:
\begin{equation}
    \mathbf{G}_{(N \times (P+1))} = \big[{R}_{(N\times 1)} \:\: \mathbf{X}_{(N\times P)} \big].
\end{equation}

Finally, we can compare the predictions of the new \textit{augmented} model in (\ref{eq:bart_synth}) with the ones of the \textit{original} BART model in (\ref{formula:BART}).
To do so, we run the two models on $b$ bootstrapped samples $b=1,...,B$ to get a set of predicted values at each iteration
\begin{eqnarray}
	\sum_{j=1}^{J} \mathcal{T}_{j,b}(\mathbf{X}; \mathcal{D}_j, \mathcal{M}_j) + \epsilon &=& \hat{Y}_{b}(\bX); \\
    \sum_{l=1}^{L} \mathcal{T}_{l,b}(\mathbf{G}; \mathcal{D}_l, \mathcal{M}_l) + \psi &=& \hat{Y}_{b}(\mathbf{G}).
\end{eqnarray}
Once we get the unit level predictions for these models at each iteration step $b$ ($\hat{y}_{b}(x_i)$ and $\hat{y}_{b}(g_i)$, respectively), we can run a series of comparisons between both the distribution of the predictions and the performance of augmented model as compared to the original model.  To assess the statistical difference between the unit level predictions' distributions we test the difference between the mean of the unit level prediction of the augmented model, $\bar{\hat{y}}(x_i)$, and the mean of the unit level predictions of the original model, $\bar{\hat{y}}(r_i)$:
\begin{eqnarray}
			\bar{\hat{y}}(x_i) &=& {1 \over B} \sum_{b=1}^{B} \hat{y}_{b}(\mathbf{X}=x_i)\\
			\bar{\hat{y}}(r_i) &=& {1 \over B} \sum_{b=1}^{B} \hat{y}_{b}(\mathbf{G}=g_i).
\end{eqnarray}	

Moreover, to assess whether or not there is an improvement in the performance of the augmented model, we run a series of tests on the difference of both the Root-Mean-Squared-Error of prediction and the adjusted $R^2$ of the two models.\footnote{For additional details on this set of tests in the online appendix.}



==> generalizability_literature.tex <==
\iffalse
These sort of issues of lack of generalizability have been largely tackled in the causal inference literature. A common instance in that stream of literature is the following: some subpopulations of interest are consistently under represented in causal inference studies and this could lead to scarce generalizability of the results. A common example is the fact that black people in the United States are much less likely to enrol in cardiovascular related clinical trials but are also though to be consistently at higher risk with respect to, say, white people. 
The streams of literature that deal with these issues are named \textit{generalizability} and \textit{transportability}. We can define both these streams of literature, following \cite{Irina Degtiar wp}, as:
(i) \textit{generalizability} refers to scenarios in which the study population is a subset of the target population (i.e., $\Omega_s \subset \Omega_t$); (ii) \textit{transportability} refers to a scenario in which the study population is external to the target population (i.e., $\Omega_s \cap \Omega_t = \o$). 
\par In the following, we will adapt these frameworks from a causal inference scenario to a scenario in which the researchers are purely interested in the quality of predictions. 
We will first introduce a set of assumptions that, we argue, are central to guarantee that the prediction of machine learning techniques are generalizable from $\Omega_s$ to $\Omega_t$. Moreover, we propose a procedure, based on a rework of the propensity score, that, we argue, is central for generalizability of predictions. Finally, we discuss in detail the Bayesian machine learning procedure, Bayesian Additive Regression Trees \citep{chipman2010bart}, that we use for the predictions in our application of financial literacy data.
Let's go back to the simple case with a study population $\Omega_s$ and a target population $\Omega_t$ that we introduced before. Let's suppose that we will use $\Omega_s$ to train a generic machine learning technique:
\begin{equation}
    Y_s = h(\bX_s) +  \psi_s,
\end{equation}
and, suppose that we want to get the predictions of $\hat{Y}_t$ using the machine learning model $h(.)$:
\begin{equation}
    \hat{Y}_t = h(\bX_t).
\end{equation}
The infeasible mean squared error for the chosen model would be the following:
\begin{equation}
    MSE^{infeas}=\mathbb{E}[(Y_{k,t}-\hat{Y}_{k,t})^2]=\mathbb{E}[(h(X_{k,t})-\hat{h}(X_{k,t}))^2],
\end{equation}
where the subscript $r$ is used to index the units in the target population (with $r=1,...,R$), while the observed mean squared error is the following:
\begin{equation}
  MSE^{obs}=\mathbb{E}[(Y_{q,s}-\hat{Y}_{q,s})^2]=\mathbb{E}[(h(X_{q,s})-\hat{h}(X_{q,s}))^2].
\end{equation}
where the subscript $q$ is used to index the units in the target population (with $q=1,...,Q$ and $Q+R=N$).
Moreover, suppose that $S_i$ is an indicator function that relates to a certain observation being in $\Omega_t$ or in $\Omega_s$: 
\begin{equation} 
    S_i=\begin{cases} 1 & \text{if} \;\;\;\;  i \in \Omega_{t}, \\ 0 & \text{otherwise}.
 \end{cases}
 \end{equation}
 We argue that to guarantee the generalizability of the predictions from $\Omega_s$ to $\Omega_t$ the following assumptions have to hold.\\
 {\textbf{Assumption 1: conditional exchangeability.}}\\
 \begin{equation}
     Y(S) \indep S \: | \: \bX,
 \end{equation}
 this assumption implies that adjusting for differences in observed predictors removes biases from comparisons between observations in the study sample and in the target sample.\\
  {\textbf{Assumption 2: positivity of selection.}}\\
 \begin{equation}
     P(S_i=1|X_i=x)>0,
 \end{equation}
this assumption states that there is a positive probability that any unit $i$ belongs to the study population given a certain set of predictors.
 %{\textbf{Assumption 3: stable unit value assumption.}}\\
 %\begin{equation}
 %    \text{If  }S_i=s \text{ then } Y_i=Y_i(s).
 %\end{equation}
We proof that if Assumption 1 and 2 hold then: \\
{\textbf{Theorem 1: convergence of the MSE}}
\begin{equation}
    MSE^{infeas} - MSE^{obs} \:\:\overset{p}{\to}\:\: 0 \:\:\: \text{as} \:\:\: N_{t} \text{ and } N_{s} \rightarrow \infty
\end{equation}
\fi
